A New Method for the Semantic Integration of Multiple OWL Ontologies using Alignments

This work is done as part of a master's thesis project. The goal is to integrate two or more ontologies (of the same or close domains) in a new consistent and coherent OWL ontology to insure semantic interoperability between them. To do this, we have chosen to create a bridge ontology that includes all source ontologies and their bridging axioms in a customized way. In addition, we introduced a new criterion for obtaining an ontology of better quality (having the minimum of semantic/logical conflicts). We have also proposed new terminology and definitions that clarify the unclear and misplaced "integration" and "merging" notions that are randomly used in state-of-the-art works. Finally, we tested and evaluated our OIA2R tool using ontologies and reference alignments of the OAEI campaign. It turned out that it is generic, efficient and powerful enough.

==> Photos/dedicace.tex <==
\chapter*{}
\thispagestyle{empty}


{\fontfamily{pzc}\selectfont
\hfill À mon papa

\hfill À ma maman

\hfill À ma sœur

\hfill À toute ma famille

\hfill Et mes amis
}
